Distributed Nonconvex Constrained Optimization over Time-Varying Digraphs

This paper considers nonconvex distributed constrained optimization over networks, modeled as directed (possibly time-varying) graphs. We introduce the first algorithmic framework for the minimization of the sum of a smooth nonconvex (nonseparable) function--the agent's sum-utility--plus a Difference-of-Convex (DC) function (with nonsmooth convex part). This general formulation arises in many applications, from statistical machine learning to engineering. The proposed distributed method combines successive convex approximation techniques with a judiciously designed perturbed push-sum consensus mechanism that aims to track locally the gradient of the (smooth part of the) sum-utility. Sublinear convergence rate is proved when a fixed step-size (possibly different among the agents) is employed whereas asymptotic convergence to stationary solutions is proved using a diminishing step-size. Numerical results show that our algorithms compare favorably with current schemes on both convex and nonconvex problems.

==> tables_nonconvex_surrogates.tex <==
\begin{table}[h]\small 
 \setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{2}
 \centering
 		\begin{tabular}{ l  l   }
 			\hline
 			Penalty function & \multicolumn{1}{l}{Expression}     \\ 
 			\hline
 			Exp \cite{bradley1998feature} & $g_{\text{exp}}(x)= 1-e^{-\theta |x|}$   \\\noalign{\smallskip}
 			
 			$\ell_p(0<p<1)$ \cite{fu1998penalized} & $g_{\ell_p^{+}}(x)= (|x|+\epsilon)^{1/\theta}$,  \\\noalign{\smallskip}
 			
 			$\ell_p(p<0)$ \cite{rao1999affine} & $g_{\ell_p^{-}}(x)= 1-(\theta |x|+1)^{p}$ \\\noalign{\smallskip}
 			 			
 			SCAD \cite{fan2001variable}& $g_{\text{scad}}(x)\!= \!\begin{cases}
 			
 			\frac{2 \theta}{a+1} |x|,  & 0 \leq |x|\leq \frac{1}{\theta}  \\
 			
 			\frac{-\theta^2 |x|^2+2 a \theta |x|-1}{a^2-1},& \frac{1}{\theta} < |x|\leq \frac{a}{\theta}  \\
 			
 			1, & |x|> \frac{a}{\theta}  \end{cases}$  \\\noalign{\smallskip}
 			
 			Log \cite{weston2003use} & $g_{\log}(x)=\frac{\log(1 +\theta |x|)}{\log(1 +\theta)}$ \\
 			
 			%Capped-$l_1$ \cite{Peleg} & $g_{cap}(t)=\min\{1,\theta |t|\}$ \medskip\\
 			
 			% PiL \cite{LeThi12} & $g_{PiL}(t)=\min\left\{1,\max\left\{0, \frac{\theta |t|-1}{a-1}\right\}\right\}$ \medskip\\
 			
 			\noalign{\smallskip}\hline
 		\end{tabular}
 		\caption{Examples of DC penalty functions satisfying \ref{assump:P3} [cf.\,(\ref{eq: dc decompose})]% $\theta >0$, $\epsilon >0$, and $a>1$.
 		}\label{tab: ncvx regularizer}  \vspace{-0.9cm}
 	\end{table} 
	 \begin{table}[h]\small 
	  \setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{2}
	 \centering
	\begin{tabular}{ l  l  l}
		\hline	 
		$g$ & $\eta(\theta)$ & \multicolumn{1}{l}{$\nabla g^{-}_{\theta}(x)$ }   \\ \noalign{\smallskip}
		 \hline 
		$g_{\textrm{exp}}$ & $\theta$ & $\text{sign}(x)\cdot\theta\cdot(1-e^{-\theta |x|})$  \\	\noalign{\smallskip}	
		$g_{\ell_p^{+}}$ &  $\frac{1}{\theta}\epsilon^{1/\theta-1}$ & $\frac{1}{\theta}\,\text{sign}(x)\cdot[\epsilon^{\frac{1}{\theta}-1}-(|x|+\epsilon)^{\frac{1}{\theta}-1}]$ \\
		
		$g_{\ell_p^{-}}$ & $-p \cdot\theta$  & $-\text{sign}(x)\cdot p\cdot \theta\cdot [1-(1+\theta |x|)^{p-1}]$ \\\noalign{\smallskip}
		
		
		$g_{\text{scad}}$ & $\frac{2 \theta}{a+1}$  & $\begin{cases}
				0,  & |x|\leq \frac{1}{\theta}  \\
				
				\text{sign}(x)\cdot \frac{2 \theta(\theta |x|-1)}{a^2-1}, & \frac{1}{\theta} < |x|\leq \frac{a}{\theta}  \\
				
				\text{sign}(x)\cdot\frac{2 \theta}{a+1}, & \text{otherwise}
		\end{cases} $\\\noalign{\smallskip}
		
		$g_{\log}$ &    $\frac{\theta}{\log(1+\theta)}$ & $\text{sign}(x)\cdot \frac{\theta^2 |x|}{\log(1+\theta)(1+\theta |x|)}$ \\
		
		%$g_{cap}$ &  $\theta$  & $\left\{ \begin{array}{lll}
		
		%0  & |x_i^{\nu}|\leq \frac{1}{\theta} \medskip \\
		
		%\text{sign}(x_i^{\nu})\theta  & \text{otherwise}  \end{array}\right.$ \medskip\\
		
		\hline\noalign{\smallskip}
	\end{tabular}
	 \caption{ Explicit expression of $\eta(\theta)$  and   $\nabla g^{-}(x)$ [cf.\,(\ref{eq: dc decompose})]   }\label{tab: gradient}\vspace{-0.2cm}
\end{table}

